Rank Overspecified Robust Matrix Recovery: Subgradient Method and Exact Recovery

We study the robust recovery of a low-rank matrix from sparsely and grossly corrupted Gaussian measurements, with no prior knowledge on the intrinsic rank. We consider the robust matrix factorization approach. We employ a robust $\ell_1$ loss function and deal with the challenge of the unknown rank by using an overspecified factored representation of the matrix variable. We then solve the associated nonconvex nonsmooth problem using a subgradient method with diminishing stepsizes. We show that under a regularity condition on the sensing matrices and corruption, which we call restricted direction preserving property (RDPP), even with rank overspecified, the subgradient method converges to the exact low-rank solution at a sublinear rate. Moreover, our result is more general in the sense that it automatically speeds up to a linear rate once the factor rank matches the unknown rank. On the other hand, we show that the RDPP condition holds under generic settings, such as Gaussian measurements under independent or adversarial sparse corruptions, where the result could be of independent interest. Both the exact recovery and the convergence rate of the proposed subgradient method are numerically verified in the overspecified regime. Moreover, our experiment further shows that our particular design of diminishing stepsize effectively prevents overfitting for robust recovery under overparameterized models, such as robust matrix sensing and learning robust deep image prior. This regularization effect is worth further investigation.

==> sections/MSNTfnorm.tex <==
In this sections we prove some facts about $\cM_t(S_t)$ and $\cN_t(T_t)$ that will be useful in the analysis.
\begin{proposition}\label{prop: bound on MM NNfnorm}
	Suppose $\gamma_t \le \frac{0.01}{\sigma_1}$,  $\norm{S_tS_t^\top - D_S^*} \le \frac{\sigma_r}{100}$, and $\norm{T_tT_t^\top}\le 0.01\sigma_r$, we have the following:
	\begin{enumerate}
		\item[1.] $\fnorm{\cM_t(S_t)\cM_t(S_t)^\top - D^*_S} \le (1-\frac{3\gamma_t\sigma_r}{4}) \fnorm{S_tS_t^\top - D_S^*} + 3 \gamma_t \fnorm{S_t T_t^\top}^2$.
		\item[2.] $\fnorm{\cN_t(T_t) \cN_t(T_t)^\top} \le  \fnorm{T_tT_t^\top}\left(1-2\gamma_t \fnorm{T_tT_t^\top}\right)$.
		\item[3.] $\fnorm{\cM_t(S_t)\cN_t(T_t)^\top} \le (1-\frac{\gamma_t\sigma_r}{3})\fnorm{S_tT_t^\top}$. 
	\end{enumerate} 
\end{proposition}

\begin{proposition}\label{prop: bound on MS NTfnorm}
Suppose $\gamma_t \le \frac{0.01}{\sigma_1}$,  $\fnorm{S_tS_t^\top - D_S^*} \le \frac{\sigma_r}{100}$, and $\fnorm{T_tT_t^\top}\le 0.01\sigma_r$, we have the following:
	\begin{enumerate}
		\item $\norm{\cN_t(T_t) S_t^\top} \le \norm{T_tS_t^\top}$.
		\item $\norm{\cN_t(T_t) T_t^\top} \le  \norm{T_t}^2(1-\gamma_t \norm{T_t}^2) = \norm{T_tT_t^\top}\left(1-\gamma_t \norm{T_tT_t^\top}\right).$
	\end{enumerate}
\end{proposition}

==> sections/algdesignanalysis_old.tex <==
In this section, we introduce the subgradient method and stepsize rule for solving \eqref{opt: main} to exact solutions. We provide the main convergence guarantee of exact recovery, and sketch the main intuitions of the proof.

%We provide the main intuition of our algorithm design, the gradient estimation via RDPP and stepsize choice, the initialization scheme, and the main theoretical guarantee of exact recovery.

\subsection{Algorithm design and analysis intuition}\label{sec: intuition}
A natural idea of optimizing the problem \eqref{opt: main} is to deploy the subgradient method starting from some initialization  $F_0\in \RR^{d\times k}$, and iterate
\begin{align}
	F_{t+1}= F_t -\eta_t g_t, \quad g_t \in \partial f(F), \,t=0,1,2,\dots. \label{eqn: algorithm}
\end{align}
 with certain stepsize rule $\eta_t\geq 0$. Here, $\partial f(F)$ is the regular subdifferential \cite{} of $f$ at point $F$, that
\begin{equation}\label{eqn: mainsubdifferential}
	\partial f(F) = \cD(FF^\top -\truX) F, \text{ where }\cD(X) := \frac{1}{m}\sum_{i=1}^{m}\sign(\dotp{A_i,X} -s_i)A_i,
\end{equation}
for any $X\in \RR^{d \times d}$. Here, the set-valued function $\sign(\cdot)$ is given by $\sign(x)=\{-1\}$ for $x<0$, $\{1\}$ for $x>0$, and $[-1,1]$ for $x=0$. 
%$\sign(x) = \begin{cases}
%	\{-1\} & x<0\\
%	[-1,1] & x=0\\
%	\{1\} & x>0
%\end{cases}$. 
%Hence the operator $\cD$  is a set-valued mapping.
 
% whose exact formula is available in \eqref{}. 

To get the main intuition of the algorithm design and analysis, let us assume for simplicity that $s_i=0$ for all $i$, i.e., $p=0$  in Models~\ref{md: randomCorruption} and \ref{md: arbitraryCorruption}, so these two models coincide. The objective $f$ in \eqref{opt: main} has expectation 
$\EE f(F)=\EE\abs {
\dotp {A_1,FF^\top-\truX}}=\sqrt{\frac{2}{\pi}}\fnorm{FF^\top -\truX}.$ Hence, we may consider a subgradient method for solving the population version $\min_{F\in \RR^{d\times k}} \EE f(F)$ :
\begin{equation}
 F_0\in \RR^{d\times k}; \qquad 
	F_{t+1}= F_t -\xi_t \underbrace{\sqrt{\frac{2}{\pi}}\frac{\left(F_tF_t^\top -\truX \right)}{\fnorm{F_tF_t^\top -\truX}}F_t}_{ = \nabla \EE f(F) \, \mid_{F=F_t}}, \;t=0,1,2,\dots. \label{eqn: sgforpop}
\end{equation}
The nondifferentiability occurs at the place where the Frobenius norm is $0$, and is problematic in the analysis. If $\xi_t\sqrt{\frac{2}{\pi}} = \gamma\fnorm{F_tF_t^\top -\truX}$ for some $\gamma>0$ always, then the above iteration scheme becomes the gradient descent for the problem $\min_{F\in \RR^{d\times k}} \fnorm{FF^\top-\truX}^2$:
\begin{equation}
 F_0\in \RR^{d\times k}; \qquad 
	F_{t+1}= F_t -\gamma\left(F_tF_t^\top -\truX \right)F_t, \;t=0,1,2,\dots. \label{eqn: gd}
\end{equation}
Analyzing the gradient decent dynamic \eqref{eqn: gd} is still possible in the rank overspecification case as recently explored in \cite{}. We defer the exact details in Section \ref{} in the appendix. 

Our main intuition for algorithm design is then to ensure the subgradient dynamic \eqref{} mimics the gradient descent dynamic \eqref{eqn: gd}. After comparing the two dynamics, we see the main task is to ensure $\eta_t g_t$ approximates $\left( F_tF_t^\top -\truX\right)F_t$ up to some multiplicative constant $\gamma$. Since $g_t$ also has a factor $F_t$ on the right as shown in \eqref{eqn: mainsubdifferential}, we only need to ensure we can approximate $F_tF_t^\top -\truX$, and we call this approximation gradient estimation.

\subsection{Gradient estimation}

We carry out the task of approximating $FF^\top -\truX$ in two steps: (1) approximating the direction $\frac{FF^\top -\truX}{\fnorm{FF^\top -\truX}}$, and (2) estimating the scale $\fnorm{FF^\top-\truX}$.\footnote{We omit the dependence on $t$ for simplicity.}
\subsubsection{Estimating the direction via RDPP}
Let us first write out the formula of the regular subdifferential of $f$:
\begin{equation}\label{eqn: mainsubdifferential}
	\partial f(F) = \cD(FF^\top -\truX) F, \text{ where }\cD(X) := \frac{1}{m}\sum_{i=1}^{m}\sign(\dotp{A_i,X} -s_i)A_i,
\end{equation}
for any $X\in \RR^{d \times d}$. Here the set-valued function $\sign$ is given by $\sign(x)=\{-1\}$ for $x<0$, $\{1\}$ for $x>0$, and $[-1,1]$ for $x=0$. 
%$\sign(x) = \begin{cases}
%	\{-1\} & x<0\\
%	[-1,1] & x=0\\
%	\{1\} & x>0
%\end{cases}$. 
Hence the operator $\cD$  is a set-valued mapping. Recall our goal here is to get an estimator of the direction $\frac{FF^\top -\truX}{\fnorm{FF^\top -\truX}}$. Since with $s_i=0$, for any $D\in \mathcal{D}(FF^\top -\truX)$ and a fixed $F$, we have $\EE[D]=\sqrt{\frac{2}{\pi}} \frac{FF^\top -\truX}{\fnorm{FF^\top -\truX}}$,  we expect 
$\cD(FF^\top -\truX)$ as a good estimate of the direction. This motivates us to define the following RDPP condition.
\ld{Liwei, somehow, I am having trouble with that RDPP applies for any $D$ in the subdifferential. In the case $\dotp{A_i,X}-s_i=0$, we have the freedom in picking a number from $[-1,1]$, what if I pick the number using other $A_i$s and $s_i$s? I think that the sign function should really be a deterministic function in the proof.}
%\qq{Here, should be $\cD(FF^\top)$ instead?}
%\ld{$y_i$ in (2.5) should really be $s_i$ Then (2.6) is right/}%\

\qq{I think here, we should introduce why RIP or other conditions not work here, and the motivations for RDPP. Discuss the relationship with $\ell_1 / \ell_2$-RIP}

\begin{definition}[RDPP]\label{defn: sign-RIP}
	The measurements and corruption $\{(A_i,s_i)\}_{i=1}^m$ are said to satisfy restricted direction preserving property with parameters $(l,\delta)$ and a scaling function $\psi: \RR^{d\times d} \rightarrow \RR$ if for every symmetric rank-$l$ matrix $X \in \RR^{d\times d}$ and every $D \in \cD(X)$, we have 
	\begin{equation}
		\norm{D - \psi(X) \frac{X}{\fnorm{X}}} \le \delta.
	\end{equation}
\end{definition}
Here the scaling function accounts for the fact that even if $s_i=0$, the population objective $\EE(f(F))= \sqrt{\frac{2}{\pi}}\fnorm{FF^\top -\truX}$, which has a pre-factor $\sqrt{\frac{2}{\pi}}$. 
\paragraph{Comparison with sign-RIP in \cite{ma2021implicit} } A \emph{major} difference between our RDPP and sign-RIP defined in \cite{ma2021implicit}  is that we use operator two norm instead of Frobenius norm there. Even though Frobenius norm is a stronger condition, unfortunately, it \emph{cannot} be satisfied even for the \emph{fixed} rank $r$ matrix $\truX$, if $m$ is on the order $dr$ as we demonstrated in Figure \ref{}.\ld{in the appendix maybe?} Since our subgradient is $g_t = DF_t$ for $D\in \mathcal{D}(FF^\top -\truX)$ with $F_t$ being low rank when $k=\mathcal{O}(r)$, it is then reasonable that $D$ approximates  $\frac{X}{\fnorm{X}}$ in operator norm is enough for our purpose. 
%Our key observation is that using the operator norm suffices for our analysis, as we only apply $\mathcal{D}(FF^\top -\truX)$ to the factor $F$ which is still low rank for $k=\mathcal{O}(r)$. \yc{I don't understand the last sentence.}

\paragraph{Relation with $\ell_1/\ell_2$ RIP}
Actually, the RDPP condition implies the $\ell_1/\ell_2$-RIP condition \eqref{} under the $p=0$ setting:
\begin{equation}
    \ld{\text{I shall write down the detail, or Liwei can fill in if you have time.}}
\end{equation}
Conversely, we know if $\ell_1/\ell_2$-RIP condition holds for all rank $d$ matrices, then RDPP holds when $s_i=0$.\cite{ma2021implicit} \ld{Does Liwei have more insights on this?}

Assuming $(r+k,\delta)$-RDPP, we see that any $D\in \mathcal{D}(FF^\top -\truX)$ is a good approximation of $\frac{FF^\top-\truX}{\fnorm{FF^\top -\truX}}$ up to the scaling factor $\psi(FF^\top -\truX)$. Next we verify that RDPP is indeed satisfied by our two models whose proof are deferred to Section \ref{sec: } in the appendix.
\begin{proposition}
RDPP is satisfied for Model \ref{md: randomCorruption}, and Model \ref{md: arbitraryCorruption}.\ld{I shall filling the detail later or Liwei can do it if you have time...}
\end{proposition}
Note that in either case the scaling function is upper and lower bounded by some positive universal constants as long as $p\leq \frac{1}{2}$. 
\subsubsection{Estimating the scale via the median and stepsize choice}
To estimate $\fnorm{FF^\top -\truX}$ under the corruption, we  define the following median operator $\tau_{\mathcal{A},y}(F):\RR^{d\times k}\rightarrow \RR$,
\begin{equation} \label{eqn: median}
 \tau_{\mathcal{A},y}(F) =\theta_{\frac{1}{2}}\left(\{|\dotp{A_i,FF^\top}-y_i|\}_{i=1}^{m}\right),
\end{equation}
where $\theta_{\frac{1}{2}}(\cdot)$ is the median operator. \ld{probably needs to be more precise here} \yc{Is the notation $o_i$ necessary?}\ld{\begin{CJK*}{UTF8}{gbsn}嗯，是不太必须。
\end{CJK*}}

We now state a proposition that ensures $\tau_{\mathcal{A},y}(F)$ approximates $\fnorm{FF^\top -\truX}$ up to a multiplicative constant under both models. The proof can be found in Section \ref{} in the appendix. Note that it is important that the approximation guarantee holds simultaneously for all $F \in \RR^{d\times k}$ since we need to apply it to the iterates which has complicated dependence on the $A_i$ and $y_i$.  
\begin{proposition}\label{prop: estimate fnorm random} Let $k\geq r$. 
 Under Model \ref{md: randomCorruption}, fix any $p<\frac{1}{2}$. Let $\epsilon = \frac{0.5-p}{3}$. Then if $m \ge c_0 dk\log d$ for some large enough constant $c_0$ depending on $p$, then with probability at least $1-c_1\exp(-c_2m\epsilon^2)- \exp(-m\epsilon^2/2)$, where $c_1$ and $c_2$ are some constants, we have for all matrix $F \in \RR^{d\times k}$ with rank at most $l$, 
	\begin{equation}
	\tau_{\mathcal{A},y}(F) \in [L_1(\epsilon), L_2(\epsilon)] \fnorm{FF^\top -\truX},
	\end{equation}
for some real valued functions $L_1,L_2$ such that $0<L_1(\epsilon)<L_2(\epsilon)<\infty$.
\yc{$\theta_{\epsilon}$ and $\theta_{1-\epsilon}$ are not defined. Do we have $\theta_{\epsilon}>0$ and $\theta_{1-\epsilon}<\infty$ and is this all we need?}\ld{\begin{CJK*}{UTF8}{gbsn}老板厉害啊！\end{CJK*}}
\yc{Notation can be improved: $F_Z$ is too similar to $F$. $\theta_\epsilon$ and $\theta_{\mathcal{A},y}$ have different meanings, so probably differentiate the notations. We may not need the notation $F_Z$, since this distribution, and hence $\theta_{\epsilon}$ and $\theta_{1-\epsilon}$ as well, never change in our paper. (Unless $\theta_{\epsilon}(F_Z)$ is something standard like the $\epsilon$ quantile of $F_Z$.)}

Under Model \ref{md: arbitraryCorruption}, fix any $\epsilon <0.1$ and $p<0.1$. Then under the same assumption on $m$ and with the same probability as above, we have
%if $m \ge c_0(\epsilon^{-2}\log \epsilon^{-1}) %dk\log d$ for some large enough constant $c_0$, %then with probability at least %$1-c_1\exp(-c_2m\epsilon^2)$, where $c_1$ and %$c_2$ are some constants, 
for any  matrix $F\in \RR^{d\times k}$,
	\begin{align}
	\tau_{\mathcal{A},y}(F)  
	%&\in [\theta_{\frac{1}{2}-p   %-\epsilon}(F_Z), %\theta_{\frac{1}{2}+p+\epsilon}(F_Z)] %\fnorm{FF^\top -\truX} \nonumber\\
		\in [L_3,(\epsilon),L_4(\epsilon)]\fnorm{FF^\top -\truX},
	\end{align}
where for some real valued functions $L_3,L_4$ such that $0<L_3(\epsilon)<L_4(\epsilon)<\infty$.
\end{proposition}

The detailed choice of $L_i(\epsilon),i=1,\dots,4$ can be found in Proposition \ref{}. They also admit the property that $\max(|L_1-L_2|,|L_3-L_4|)\rightarrow 0$ as $\epsilon\rightarrow 0$. \ld{Liwei, is the approaching 0 statement true? can you make it clear in Section \ref{sec: Choice of Stepsize}?}  Note for the arbitrary corruption Model~\ref{md: arbitraryCorruption}, we require a more stringent condition $p<0.1$, while in Model~\ref{md: randomCorruption}, we allow $p$ to be close to $\frac{1}{2}$. \ld{it looks like for model 1, even if p is small, the interval in (3.6) does not shrink to 0, why is that, Liwei? We also need a definition on $\theta_{\epsilon}$ or some substitute.}  \lj{The reason is that I simply picked a constant $\epsilon$ in that proposition. We can make the interval small by choosing a smaller $\epsilon$. Do you want me to make the change? The notation was simply borrowed from Yuejie's paper}

Hence to choose the stepsize, we use the following adaptive stepsize rule: pick a $\gamma>0$ and set the stepsize 
\begin{equation}\label{eqn: stepsizerule}
    \eta_t = \gamma \theta_{\mathcal{A},y}(F_t).
\end{equation}
This choice of stepsize with RDPP and previous proposition ensure that indeed 
$
\eta_t g_t$ indeed approximates $(F_tF_t^\top -\truX)F$
well.


\subsection{Initialization scheme}

We have specified the stepsize rule \eqref{eqn: stepsizerule}. To ensure algorithmic success of \eqref{eqn: algorithm}, another important missing piece is the choice of the initialization $F_0$. Here we propose an spectral method as Algorithm \ref{}. 

The algorithm \ref{} is basically taking the top $k$ SVD of the matrix $-D$ where $D\in \mathcal{D}(-\truX))$.\yc{This is over-simplification: we don't know $\truX$ and estimating $\truX$ is the problem to begin with.}\ld{\begin{CJK*}{UTF8}{gbsn}我弄错了 不好意思\end{CJK*}} Now we state an guarantee of it. Note that because scale information is missing, we should really compare it to the the scaled $\psi(\truX)\frac{\truX}{\fnorm{\truX}}$. Our guarantees is stated as the following proposition whose proof can be found in Section \ref{} in the appendix.
\begin{proposition}
 \ld{\text{a proposition for both models but comparing to the scaled $\truX$}}
\end{proposition}
Note that we only require the direction to be accurate instead of the usual condition that $\norm{F_0F_0-\truX}$ to be small \cite{} or even $\fnorm{F_0F_0^\top -\truX}$ to be small \cite{}. 
As we shall see in the next section, direction accuracy combined with a rough estimate of the scale $\fnorm{\truX}$, which can be obtained by $\theta_{\mathcal{A},y}(0)$, is enough for our initialization purpose. In particular, we compute an initial solution by
\begin{equation}\label{eqn: intialization}
 F_0 = \theta_{\mathcal{A},y}(0) \hat{B},
\end{equation}
where $\hat{B}$ is the output of Algorithm \ref{}. 
Such a weak requirement on the initialization is the key that allows for $p$ to be close to $\frac{1}{2}$ in the Model \ref{md: randomCorruption} case.\footnote{The work 
\cite{} 
actually allows for $p$ to be close to $1$, albeit its guarantee only applies to $r=1$ and is only approximately recovery, $\norm{F_0F_0^\top -\truX}\leq \delta$ for their initialization scheme \cite[Algorithm 2]{} under a sign-RIP condition. Unfortunately, as mentioned in Section {}, their sign-RIP condition does not hold for $m=\mathcal{O}(dk)$. Even worse, in their Algorithm 2, the scale information $\fnorm{\truX}$ is known a priori and used. However, estimating $\fnorm{\truX}$ accurately requires $p$ to be close to $0$. } A guarantee of similar flavor as the past, e.g., small $\norm{F_0F_0^\top -\truX}$, can be obtained as well for $p$ small enough, which we defer to the appendix. We point out that this kind initialization guarantee also meets our initialization requirement even though our requirement is much weaker. 



\subsection{Main Theoretical guarantee}

\qq{I think maybe we should put this subsection before Section 3.2? The readers often want to see the result first because looking at these lengthy analysis.}\ld{\begin{CJK*}{UTF8}{gbsn}也是可以的。但有点蛋疼。移到前面的话需要refer一些后面section的概念\end{CJK*}}

In this section, we show that our subgradient method \eqref{eqn: algorithm} equipped with the initialization scheme  \eqref{eqn: intialization} and our adaptive stepsize choice  \eqref{eqn: stepsizerule} ensures that the iterate $F_tF_t^\top$ converges to $\truX$. 

Our first lemma articulates the condition that ensures the convergence of the subgradient method \eqref{eqn: algorithm}:
\begin{lem}\label{lem: mainlemma}
Suppose the following condition holds:
(i) $(r+k,\delta)$-RDPP holds for $\{A_i,s_i\}_{i=1}^m$ with $\delta \leq ?$;
(ii) the initialization $F_0 = \alpha B$ satisfies that $c_1\fnorm{\truX}\leq \alpha^2\leq c_2\fnorm{\truX}$ for some numerical constant $c_1,c_2>0$. and $\norm{BB^\top -\psi(\truX)\frac{\truX}{\fnorm{\truX}}}\leq ?$; (iii) the step size $\xi c_1\leq \frac{\eta_t\fnorm{F_tF_t^\top -\truX}}{\psi(F_tF_t^\top -\truX} \leq \xi c_2$ for some small numerical constant $\xi$ and all $t$. Then for $k\geq r$, if $t \ge \mathcal{T}:= \kappa \log $, we have 
\[
\norm{F_tF_t^\top -\truX} \leq ?.
\]
Moreover, if $k=r$, then under the same set of condition, we have for $t\geq \mathcal{T}$
\[
\norm{F_tF_t^\top -\truX} \leq ?.
\]
\end{lem} 
\begin{proof}[Proof sketch]
Apart from the intuition that the subgradient dynamics \eqref{eqn: algorithm} mimics the gradient dynamic \eqref{eqn: gd}, which is ensured by condition (i) and (iii) above, another idea in the proof is that we need to decompose the iterate $F_t$ into two parts as done in \cite{}.
Let the singular value decomposition of $\truX$ be 
\begin{equation}
	\truX = \begin{bmatrix}
		U & V
	\end{bmatrix}\begin{bmatrix}
		D_S^* & 0\\
		0   & 0
	\end{bmatrix}
	\begin{bmatrix}
		U & V
	\end{bmatrix}^\top,
\end{equation}
where $U \in \RR^{d\times r}, V \in \RR^{d \times d-r}, D_S^* \in \RR^{r \times r}$. $U$ and $V$ has orthonormal columns and $U^\top V = 0$. Since union of column space of $U$ and $V$ spans the whole space, for any $F_t \in \RR^{d\times r}$, we can write 
\begin{equation}
	F_t = US_t + VT_t,
\end{equation} 
where $S_t = U^\top F_t \in \RR^{r \times k}$ and $T_t = V^\top F_t \in \RR^{(d-r)\times k}$. Unlike the proof in \cite{}, we need to deal with the initialization stage where $\norm{F_tF_t^\top-\truX}$ are still very large. Recall our condition (ii) only ensures that the initial $F_0F_0^\top$ is only accurate up to some scaling factor. To deal with this issue, our proof is split into three stages: (i) showing that the smallest singular value of $S$ increases, (ii) the differences $SS^\top-D$, $ST$, decrease geometrically. This is why we have a burn-in phase $T$. In stage (iii), due to sublinear convergence of $TT^\top$, we have the sublinear rate of $F_tF^\top_t$. If $k=r$, then we have a better control of $TT^\top$ and the method converges geometrically as well, and that's why we have a speed up for $k=r$. 
\yc{$T$ is used to denote both a matrix (the signal part) and a number (the burn-in iteration).}\ld{\begin{CJK*}{UTF8}{gbsn}你说的对\end{CJK*}}
\end{proof}

Equipped with Lemma~\ref{lem: mainlemma}, we now state our main theorem.
\begin{thm}
Suppose under Model \ref{md: randomCorruption}, we have $m\geq $ and $p<\frac{1}{2}-\epsilon$ for some small numerical constant $\epsilon$, and under Model \ref{md: arbitraryCorruption}, we have $m\geq$ and $p$. Then under both models, our subgradient method \eqref{eqn: algorithm} with the initialization scheme \eqref{eqn: intialization} and the adaptive stepsize choice \eqref{eqn: stepsizerule} for some small numerical constant $\gamma>0$, we have for $k\geq r$, and $t\geq \mathcal{T}$
\[
\norm{F_tF_t^\top -\truX} \leq ?.
\]
Moreover, if $k=r$, then under the same set of condition, we have for $t\geq \mathcal{T}$
\[
\norm{F_tF_t^\top -\truX} \leq ?.
\]
\yc{Do the above require $t\ge T$?}
\end{thm}\ld{\begin{CJK*}{UTF8}{gbsn}老板你说的对\end{CJK*}}
\begin{proof}
verify each condition in Lemma \ref{lem: mainlemma}.
\end{proof}
\ld{Liwei, can you fill in the details of the theorems, lemma, and proposition, and above proof?}
We would like to reemphasize that it is because our weak initialization condition, we are allowed to take $p$ to be close to $\frac{1}{2}$ in the model \ref{md: randomCorruption} setting.


==> sections/analysisfnorm.tex <==

First of all, our initialization strategy will give us the following initialization quality.
\begin{proposition}[Initialization quality]\label{prop: initialization quality fnorm}
	Under our initialization, we have 
   \begin{equation}
   	\krnorm{F_0F_0^\top -X^*}=\fnorm{F_0F_0^\top -X^*} \le \frac{\sigma_r}{100}.
   \end{equation}
Moreover,
\begin{align}
	\fnorm{S_0S_0^\top -D_S^*} &= \krnorm{S_0S_0^\top - D_S^*} \le \frac{\sigma_r}{100},\\
	\fnorm{S_0T_0^\top} &= \krnorm{S_0T_0^\top} \le \frac{\sigma_r}{100},\\
	\fnorm{T_0T_0^\top} &= \krnorm{T_0T_0^\top} \le \frac{\sigma_r}{100}.
\end{align}
\end{proposition} 
\noindent The next proposition illustrates the evolution of $S_t$ and $T_t$.
\begin{proposition}[Updates of $S_t,T_t$]\label{prop: updates of S,T}
	For any $t \ge 0$, we have 
	\begin{align}
		S_{t+1} &= S_t - \gamma_t\left(S_t S_t^\top S_t + S_t T_t^\top T_t -D_S^*S_t\right) + \gamma_t U^\top \Delta_t F_t,\\
		T_{t+1} &= T_t - \gamma_t \left(T_tT_t^\top T_t + T_tS_t^\top S_t \right) + \gamma_t V^\top \Delta_t F_t.
	\end{align}
\end{proposition}
We introduce notations
\begin{align}
	\cM_t(S_t) &= S_t- \gamma_t\left(S_t S_t^\top S_t + S_t T_t^\top T_t -D_S^*S_t\right) \\
	\cN_t(T_t) &= T_t - \gamma_t \left(T_tT_t^\top T_t + T_tS_t^\top S_t \right).
\end{align}
They are "population-level" updates for $S_t$ and $T_t$, in the sense that 
\begin{align}
	\cM_t(S_t) &= U^\top \left(F_t - \gamma_t(F_tF_t^\top - X^*) \right),\\
	\cN_t(T_t) &= T^\top \left(F_t - \gamma_t(F_tF_t^\top - X^*) \right).
\end{align}
So $\cM_t(S_t)$ and $\cN_t(T_t)$ has rank at most $k$.
The analysis consists of two stages:
\begin{itemize}
	\item In stage $1$, we show that $D_t=\max\{\fnorm{S_tS_t^\top - D_S^*}, \fnorm{S_tT_t^\top}\}$ decreases geometrically if it is bigger than $10\delta \sigma_1$, which is the computational threshold. In other words, $\fnorm{S_tS_t^\top - D_S^*}$ decrease to a $10\delta \sigma_1$ geometrically, and this will happen by $\cT$.
	\item  In stage $2$, after $\cT$, $E_t =\max\{\fnorm{S_tS_t^\top - D_S^*}, \fnorm{S_tT_t^\top},\fnorm{T_tT_t^\top}\}$ converges to $0$ sublinearly. 
\end{itemize} 
In the above statement,
\begin{equation}
\cT= \ceil{\frac{\log\left( \frac{1000\delta \sigma_1}{\sigma_r}\right)}{\log\left(1-\frac{c_\gamma(1-p)\sigma_r}{6}\right)}} 
\end{equation}
Stage $1$ consists of all the iterations up to time $\cT$.  Stage $2$ consists of all the iterations afterwards.

==> sections/analysisopnorm.tex <==

First of all, our initialization strategy will give us the following initialization quality.
\begin{proposition}[Initialization quality]\label{prop: initialization quality}
	Under our initialization, we have 
	\begin{align}
		4\norm{T_0}^2 &\le 0.001\sigma_r(S_0) \frac{\sigma_r}{\sqrt{\sigma_1}}\\
		\norm{T_0}&\le \min\{0.1\sqrt{\sigma_1},\frac{\sigma_r}{200\sqrt{\sigma_1}}\}=\frac{\sigma_r}{200\sqrt{\sigma_1}}\\
		\norm{S_0} &\le 2\sqrt{\sigma_1}.
	\end{align}
In the analysis, we will let 
	\begin{align}
		\sigma_r(S_0) &= \rho\\
		\norm{T_0} &=c_\rho \rho\\
		\norm{S_0} & \le 2\sqrt{\sigma_1}.
	\end{align}
The parameters satisfy $4(c_\rho\rho)^2 \le 0.001 \rho \frac{\sigma_r}{\sqrt{\sigma_1}}$ and $c_\rho \rho \le \min\{0.1\sqrt{\sigma_1},\frac{\sigma_r}{200\sqrt{\sigma_1}} \}=\frac{\sigma_r}{200\sqrt{\sigma_1}}$.
\end{proposition} 
\noindent The next proposition illustrates the evolution of $S_t$ and $T_t$.
\begin{proposition}[Updates of $S_t,T_t$]\label{prop: updates of S,T}
	For any $t \ge 0$, we have 
	\begin{align}
		S_{t+1} &= S_t - \gamma_t\left(S_t S_t^\top S_t + S_t T_t^\top T_t -D_S^*S_t\right) + \gamma_t U^\top \Delta_t F_t,\\
		T_{t+1} &= T_t - \gamma_t \left(T_tT_t^\top T_t + T_tS_t^\top S_t \right) + \gamma_t V^\top \Delta_t F_t.
	\end{align}
\end{proposition}
We introduce notations
\begin{align}
	\cM_t(S_t) &= S_t- \gamma_t\left(S_t S_t^\top S_t + S_t T_t^\top T_t -D_S^*S_t\right) \\
	\cN_t(T_t) &= T_t - \gamma_t \left(T_tT_t^\top T_t + T_tS_t^\top S_t \right).
\end{align}
They are "population-level" updates for $S_t$ and $T_t$, in the sense that 
\begin{align}
	\cM_t(S_t) &= U^\top \left(F_t - \gamma_t(F_tF_t^\top - X^*) \right),\\
	\cN_t(T_t) &= T^\top \left(F_t - \gamma_t(F_tF_t^\top - X^*) \right).
\end{align}
So $\cM_t(S_t)$ and $\cN_t(T_t)$ has rank at most $k$.
\begin{proposition}[Uniform upper bound]\label{prop: uniform upper bound}
	Suppose $\gamma_t$ satisfies $\gamma_t \le \frac{0.01}{\sigma_1}$ for all $t\ge 0$ and $ (50\sqrt{k}\delta)^{\frac{1}{3}} \le \frac{c_\rho\rho}{2\sqrt{\sigma_1}} $, we have 
	\begin{align}
		\norm{T_t} &\le (c_\rho \rho)^\frac{1}{2}\le 0.1 \sqrt{\sigma_r}\le 0.1 \sqrt{\sigma_1}\\
		\norm{S_t} &\le 2 \sqrt{\sigma_1}
	\end{align}
for all $t \ge 0$.
\end{proposition}
The analysis consists of three stages:
\begin{itemize}
	\item In stage $1$, we show at $\sigma_r(S_t)$ increases geometrically to level $\sqrt{\frac{\sigma_r}{2}}$ by time $\cT_1'$, then $\norm{S_tS_t^\top - D_S^*}$ will decrease geometrically to $\frac{100(c_\rho \rho)^2\sigma_1}{\sigma_r}(\le \frac{\sigma_r}{100})$by $\cT_1$. The iterate will then enter a good region.
	\item In stage $2$, we show that $D_t=\max\{\norm{S_tS_t^\top - D_S^*}, \norm{S_tT_t^\top}\}$ decreases geometrically if it is bigger than $10\delta \sqrt{k+r}\sigma_1$, which is the computational threshold. In other words, $\norm{S_tS_t^\top - D_S^*}$ decrease to $10\delta \sqrt{k+r}\sigma_1$ geometrically, and this will happen by $\cT_2$.
	\item  In stage $3$, after $\cT_2$, $E_t =\max\{\norm{S_tS_t^\top - D_S^*}, \norm{S_tT_t^\top},\norm{T_tT_t^\top}\}$ converges to $0$ sublinearly. 
\end{itemize} 
In the above statement, \begin{equation}
	\cT_1' = \ceil{\log \left(\frac{\sqrt{\sigma_r}}{\sqrt{2}\rho}\right)/ \log\left(1+\frac{c_\gamma\sigma_r(1-p)}{6}\right)},
\end{equation} 
\begin{equation}
	\cT_1= \cT_1' + \ceil{\frac{\log(\frac{20  (c_\rho \rho)^2}{\sigma_r})}{\log\left(1- \frac{c_\gamma (1-p)\sigma_r}{2}\right)}}
\end{equation}
and 
\begin{equation}
	\cT_2= \cT_1 + \ceil{\frac{\log\left( \frac{1000\delta \sqrt{k+r}\sigma_1}{\sigma_r}\right)}{\log\left(1-\frac{c_\gamma(1-p)\sigma_r}{6}\right)}}.
\end{equation}
Stage $1$ consists of all the iterations up to time $\cT_1$. Stage $2$ consists of all the iterations between $\cT_1 + 1$ and $\cT_2$. Stage $3$ consists of all the iterations afterwards.

==> sections/neuripschecklist.tex <==
 
\begin{enumerate}

\item  For all authors...
\begin{enumerate}
    \item \textit{Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?} \answerYes{Our contribution is stated in the introduction and the abstract. A paragraph ``Our approach and contributions" states our contributions in detail. We briefly mentioned our assumptions in the introduction and abstract, and described in detail in Section \ref{sec:models}. We also verify the claims in our numeric section, Section \ref{sec:exp}.}
\item\textit{Have you read the ethics review guidelines and ensured that your paper conforms to them?} \answerYes{}

\item\textit{Did you discuss any potential negative societal impacts of your work?} \answerNo{We did not discuss potential negative societal impacts of our work in the main text as it may blur the main message we want to convey, and our work is about providing firm foundation for machine learning algorithms instead of direct applications.

We expect that this work has very limited implications for fairness, interpretability, and related topics,
as it merely provides theoretical foundations for 
algorithms advance for matrix factorization problems. However, we do note that our algorithm may enhance certain decision making when the problem pertains to socially important applications.}

\item \textit{Did you describe the limitations of your work?}
\answerYes{The limitations of the current work are included in the section \ref{sec: conclusion}.}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
    \item  \textit{Did you state the full set of assumptions of all theoretical results?} \answerYes{We state our model assumptions in Section \ref{sec:models}. For each lemma, proposition, theorem, we stated additional assumptions needed in the lemma, proposition, theorem statement. }

\item \textit{Did you include complete proofs of all theoretical results?} \answerYes{All proofs are included in the supplement. We give references for theorems without proof. }

\end{enumerate}

\item If you ran experiments...

\begin{enumerate}
    \item \textit{Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?} \answerYes{Our experiment is more on the ``proof of concept'' type of experiments. Nevertheless, we provide enough details in the section \ref{sec:exp} and in the supplement to reproduce the result.}

\item \textit{Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?} \answerYes{}

\item \textit{Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?} \answerNo{As mentioned, our experiment is really just ``proof of concept'' type experiments. We have checked the performance for multiple random seeds already. }

\item \textit{Did you include the amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?} \answerYes{They are all included in the supplement.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{This is mentioned in footnote 9, in page 9.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{We cited \cite{BM3D} and obtained the license therein for the usage of data, which is publicly available for academic usage.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> sections/stageonefnorm.tex <==
 Define 
\begin{equation}
	D_t = \max\{\fnorm{S_t S_t^\top- D_S^*}, \fnorm{S_t T_t^\top}\}.
\end{equation} 
We show that $D_t$ decreases to $100\delta\sigma_1$ geometrically after $\cT_1$.
\begin{proposition}\label{prop: stagetonefnorm}
	Suppose there is some constant $c_\gamma>0$ such that the parameters satisfy $c_\gamma(1-p)\le \gamma_t \le \frac{0.01}{\sigma_1}$, $ \delta \le \frac{0.001\sigma_r}{\sigma_1}$. Also, we suppose $\fnorm{T_tT_t^\top}\le 0.01\sigma_r$ for all $t$. 
 Then For any $t\ge 0$, we have
	\begin{equation}\label{eqn: stageonefnorm}
		D_{\cT_1 +t} \le \max\left\{\left(1-\frac{c_\gamma(1-p)\sigma_r}{6}\right)^t\cdot \frac{\sigma_r}{100} ,10\delta \sqrt{2k} \sigma_1\right\}.
	\end{equation}
	In particular, Proposition~\ref{prop: stagetwofnorm} will imply that $\fnorm{T_tT_t^\top}\le 0.01\sigma_r$ for all $t$, so for $\cT= \ceil{\frac{\log\left( \frac{1000\delta \sigma_1}{\sigma_r}\right)}{\log\left(1-\frac{c_\gamma(1-p)\sigma_r}{6}\right)}} $, we have 
	\begin{align}
		\norm{S_t S_t^\top - D_S^*} &\le 10\delta \sqrt{k}\sigma_1,\\ 
		\norm{S_t T_t^\top} &\le 10\delta \sqrt{k}\sigma_1, \qquad \forall t \ge \cT.
	\end{align}
\end{proposition}

==> sections/stagetwofnorm.tex <==
Define 
\begin{equation}
	E_t = \max\{\fnorm{S_tS_t^\top -D_S^*}, \fnorm{S_t T_t^\top}, \fnorm{T_tT_t^\top}\}.
\end{equation} 
We are going to show the sublinear convergence of $E_t$ in stage three.
\begin{proposition}\label{prop: stagetwofnorm}
	Suppose we have $\gamma_t \le \frac{0.01}{\sigma_1}$, $\delta\sqrt{2k} \le \frac{0.001 \sigma_r}{\sigma_1}$ and $E_{t} \le 0.01\sigma_r$ for some $t>0$. Then we have
	\begin{equation}
		E_{t+1} \le  \max \{(1-\frac{\gamma_t\sigma_r}{6})E_t, E_t(1-\gamma_t E_t)\} =E_t(1-\gamma_tE_t).
	\end{equation}
\end{proposition}
